Efficient Continual Learning with Modular Networks and Task-Driven Priors

Existing literature in Continual Learning (CL) has focused on overcoming catastrophic forgetting, the inability of the learner to recall how to perform tasks observed in the past. There are however other desirable properties of a CL system, such as the ability to transfer knowledge from previous tasks and to scale memory and compute sub-linearly with the number of tasks. Since most current benchmarks focus only on forgetting using short streams of tasks, we first propose a new suite of benchmarks to probe CL algorithms across these new axes. Finally, we introduce a new modular architecture, whose modules represent atomic skills that can be composed to perform a certain task. Learning a task reduces to figuring out which past modules to re-use, and which new modules to instantiate to solve the current task. Our learning algorithm leverages a task-driven prior over the exponential search space of all possible ways to combine modules, enabling efficient learning on long streams of tasks. Our experiments show that this modular architecture and learning algorithm perform competitively on widely used CL benchmarks while yielding superior performance on the more challenging benchmarks we introduce in this work.

==> img/long_stream_100.tex <==
\begin{tabular}{lp{1cm}p{1cm}p{1cm}p{1cm}}
\toprule
{} &  $<\mathcal{A}>$ &  $<\mathcal{F}>$ &   Mem. &  FLOPs \\
Model       &                  &                  &        &        \\
\midrule
Independent &             0.55 &             0.00 &  243.7 &   3088 \\
Finetune    &             0.20 &            -0.34 &    2.4 &   4780 \\
Online EWC  &             0.25 &            -0.24 &    7.4 &   4259 \\
MNTDP-D     &             0.75 &             0.00 &   99.9 &  23359 \\
\bottomrule
\end{tabular}


==> tables/AverageAcc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{ccccc}
\hline
\textbf{Dataset}                                                                    & \textbf{Model} & \textbf{Acc} & \textbf{\# Params} & \textbf{Avg FLOPs per task} \\ \hline
\multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}Split Cifar 10\\ 5 tasks\end{tabular}}   & Inde           & 97.08        & 3.5M               &                             \\
                                                                                    & Multi-head     & 69.18        & 1.9M               &                             \\
                                                                                    & Multi-leg      & 68.8         & 0.7M               &                             \\ \cline{2-5} 
                                                                                    & EWC            &              &                    &                             \\
                                                                                    & ER             &              &                    &                             \\
                                                                                    & PNN            &              &                    &                             \\
                                                                                    & RPSNet         &              &                    &                             \\ \cline{2-5} 
                                                                                    & Ours           &              &                    &                             \\ \hline
\multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}Split Cifar 100\\ 10 tasks\end{tabular}} & Inde           & 82.45        & 7.02M              &                             \\
                                                                                    & Multi-head     & 46.17        & 3.4M               &                             \\
                                                                                    & Multi-leg      & 18.84        & 0.7M               &                             \\ \cline{2-5} 
                                                                                    & EWC            &              &                    &                             \\
                                                                                    & ER             &              &                    &                             \\
                                                                                    & PNN            &              &                    &                             \\
                                                                                    & RPSNet         &              &                    &                             \\ \cline{2-5} 
                                                                                    & Ours           &              &                    &                             \\ \cline{2-5} 
\end{tabular}
\caption{\label{tab:avg-acc}Average accuracy after training on all tasks.}
\end{table}

==> tables/long_stream_probas.tex <==
\begin{table}[]
\centering
\begin{tabular}{cccc}
\hline
\textbf{Tasks ids} & 0-32 & 33-66 & 67-100 \\ \hline
$P(large)$ & 0.5  & 0.25  & 0      \\
$P(small)$ & 0.5  & 0.75  & 1      \\ \hline
\end{tabular}
\caption{\label{tab:long-stream-probas}Detail of the different data
  regimes for the generation of the long stream. \mr{Does this have
    100 or 101 tasks? Please, check the intervals in the table and
    make the consistent with the main text.} \mr{Why do we need this
    table? It's just 3 numbers that we need to report, no?}}
\end{table}


==> tables/plasticity.tex <==
\begin{tabular}{lcccccc}
\toprule
{} &  Acc $T_5$ &  $<\mathcal{A}>$ &  $<\mathcal{F}>$ &   Mem. &  FLOPs &  LCA@5 \\
\textbf{Model            } &            &                  &                  &        &        &        \\
\midrule
\textbf{Independent      } &       0.71 &             0.59 &             0.00 &  12.19 &    232 &   0.10 \\
\textbf{Finetune         } &       0.57 &             0.21 &            -0.30 &   2.44 &    274 &   0.12 \\
\textbf{New-head freeze  } &       0.29 &             0.45 &             0.00 &   2.45 &    294 &   0.13 \\
\textbf{New-head finetune} &       0.56 &             0.20 &            -0.35 &   2.45 &    336 &   0.11 \\
\textbf{New-leg freeze   } &       0.27 &             0.37 &             0.00 &   2.47 &    390 &   0.10 \\
\textbf{New-leg finetune } &       0.58 &             0.19 &            -0.34 &   2.47 &    375 &   0.11 \\
\textbf{EWC              } &       0.28 &             0.27 &            -0.19 &  26.69 &    239 &   0.11 \\
\textbf{Online EWC       } &       0.28 &             0.30 &            -0.17 &   7.29 &    282 &   0.12 \\
\textbf{ER (Reservoir)   } &       0.48 &             0.20 &            -0.27 &  11.66 &    383 &   0.10 \\
\textbf{ER               } &       0.51 &             0.45 &            -0.08 &  11.66 &    597 &   0.10 \\
\textbf{PNN              } &       0.56 &             0.54 &             0.00 &  36.50 &   1742 &   0.13 \\
\textbf{MNTDP-S          } &       0.58 &             0.55 &             0.00 &  10.98 &    351 &   0.10 \\
\textbf{MNTDP-S (k=all)  } &       0.60 &             0.56 &             0.00 &  10.98 &    340 &   0.11 \\
\textbf{MNTDP-D          } &       0.70 &             0.62 &             0.00 &  11.58 &   1503 &   0.10 \\
\bottomrule
\end{tabular}


==> tables/res/cifar_split.tex <==
\begin{tabular}{lcccc}
\toprule
{} &  $<\mathcal{A}>$ &  $<\mathcal{F}>$ &    Mem. &    FLOPs \\
\textbf{Model            } &                  &                  &         &          \\
\midrule
\textbf{Independent      } &             0.82 &             0.00 &   24.39 &  1327.16 \\
\textbf{Finetune         } &             0.18 &            -0.56 &    2.44 &   886.03 \\
\textbf{New-head freeze  } &             0.57 &             0.00 &    2.46 &   739.61 \\
\textbf{New-head finetune} &             0.21 &            -0.52 &    2.46 &   687.05 \\
\textbf{New-leg freeze   } &             0.50 &             0.00 &    2.51 &  1758.91 \\
\textbf{New-leg finetune } &             0.18 &            -0.42 &    2.51 &  1115.04 \\
\textbf{EWC              } &             0.55 &             0.01 &   50.96 &  1150.84 \\
\textbf{Online EWC       } &             0.54 &            -0.02 &    7.30 &  1053.12 \\
\textbf{ER (Reservoir)   } &             0.32 &            -0.50 &   20.90 &  1742.02 \\
\textbf{ER               } &             0.66 &            -0.15 &   20.90 &  1524.27 \\
\textbf{PNN              } &             0.78 &             0.00 &  133.76 &  9888.96 \\
\textbf{MNTDP-S          } &             0.75 &             0.00 &   24.39 &  1295.25 \\
\textbf{MNTDP-S (k=all)  } &             0.75 &             0.00 &   24.37 &  1323.41 \\
\textbf{MNTDP-D          } &             0.83 &             0.00 &   24.34 &  6168.40 \\
\bottomrule
\end{tabular}




==> tables/res/long_stream_50.tex <==


 % Result using mixed_all 60 strategy from exp defaultdict(<class 'list'>, {333262031: [2584, 2625]}) - 2584 2625
\begin{tabular}{lcccccccccccc}
\toprule
{} & \multicolumn{2}{l}{Acc $T_1$} & \multicolumn{2}{l}{$Acc_T$} & \multicolumn{2}{l}{$Acc_t$} & \multicolumn{2}{l}{Steps (K)} & \multicolumn{2}{l}{Params (M)} & \multicolumn{2}{l}{LCA} \\
{} &      mean & std &    mean & std &    mean & std &      mean & std &       mean & std &      mean & std \\
\textbf{Model            } &           &     &         &     &         &     &           &     &            &     &           &     \\
\midrule
\textbf{Independent      } &      0.72 &   - &    0.58 &   - &    0.58 &   - &     20.95 &   - &      36.56 &   - &  0.203412 &   - \\
\textbf{Finetune         } &         - &   - &       - &   - &       - &   - &         - &   - &          - &   - &         - &   - \\
\textbf{New-head freeze  } &         - &   - &       - &   - &       - &   - &         - &   - &          - &   - &         - &   - \\
\textbf{New-head finetune} &         - &   - &       - &   - &       - &   - &         - &   - &          - &   - &         - &   - \\
\textbf{New-leg freeze   } &         - &   - &       - &   - &       - &   - &         - &   - &          - &   - &         - &   - \\
\textbf{New-leg finetune } &         - &   - &       - &   - &       - &   - &         - &   - &          - &   - &         - &   - \\
\textbf{EWC              } &         - &   - &       - &   - &       - &   - &         - &   - &          - &   - &         - &   - \\
\textbf{Online EWC       } &         - &   - &       - &   - &       - &   - &         - &   - &          - &   - &         - &   - \\
\textbf{ER (Reservoir)   } &         - &   - &       - &   - &       - &   - &         - &   - &          - &   - &         - &   - \\
\textbf{ER (Ring Buffer) } &         - &   - &       - &   - &       - &   - &         - &   - &          - &   - &         - &   - \\
\textbf{PNN              } &         - &   - &       - &   - &       - &   - &         - &   - &          - &   - &         - &   - \\
\textbf{NAS-S beam=1     } &         - &   - &       - &   - &       - &   - &         - &   - &          - &   - &         - &   - \\
\textbf{NAS-S full       } &         - &   - &       - &   - &       - &   - &         - &   - &          - &   - &         - &   - \\
\textbf{NAS-D            } &      0.72 &   - &    0.75 &   - &    0.75 &   - &    148.13 &   - &      17.06 &   - &  0.305106 &   - \\
\bottomrule
\end{tabular}





==> tables/res_cifar.tex <==
\begin{table}[]
\begin{center}
\begin{tabular}{clccc}
\hline
\textbf{Stream}                                                                     & \multicolumn{1}{c}{\textbf{Model}} & \textbf{Avg Acc}     & \textbf{\# Params}   & \textbf{\# Steps}    \\ \hline
\multirow{10}{*}{\begin{tabular}[c]{@{}c@{}}Split Cifar 100\\ 20 tasks\end{tabular}} & EWC                                &                      &                      &                      \\
                                                                                     & ER                                 &                      &                      &                      \\
                                                                                     & Finetune                           &                      &                      &                      \\
                                                                                     & Inde                               & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \cline{2-5} 
                                                                                     & New-head FT                        &                      &                      &                      \\
                                                                                     & New-head freeze                    &                      &                      &                      \\
                                                                                     & PNN                                &                      &                      &                      \\
                                                                                     & P\&C                               &                      &                      &                      \\ \cline{2-5} 
                                                                                     & Nas-D                              & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
                                                                                     & Nas-S                              &                      &                      &                      \\ \hline
\multirow{10}{*}{\begin{tabular}[c]{@{}c@{}}Split Cifar 100\\ 10 tasks\end{tabular}} & EWC                                &                      &                      &                      \\
                                                                                     & ER                                 &                      &                      &                      \\
                                                                                     & Finetune                           &                      &                      &                      \\
                                                                                     & Inde                               & 82.45                & 7.02M                &                      \\ \cline{2-5} 
                                                                                     & New-head FT                        &                      &                      &                      \\
                                                                                     & New-head freeze                    &                      &                      &                      \\
                                                                                     & PNN                                &                      &                      &                      \\
                                                                                     & P\&C                               &                      &                      &                      \\ \cline{2-5} 
                                                                                     & Nas-D                              & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
                                                                                     & Nas-S                              & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \hline
\end{tabular}

\caption{\label{tab:res-cifar}Results on the standard 10 tasks and 20 tasks version of the split Cifar 100 stream. 
}

\end{center}
\end{table}

==> tables/res_long_stream_25.tex <==
\begin{table}[]
\begin{center}

% Result using mixed_all 25 strategy from exp defaultdict(<class 'list'>, {295880737: [2301, 2304]}) - 2301 2304
\begin{tabular}{lcccccc}
\toprule
{} &            Acc $T_1$ &              Avg acc &    Avg acc when seen &            Total steps &              Total params &  LCA \\
Model                &                      &                      &                      &                        &                           &      \\
\midrule
EWC                  &                    - &                    - &                    - &                      - &                         - &    - \\
Experience Replay    &                    - &                    - &                    - &                      - &                         - &    - \\
Finetune             &  0.792 $\pm$ 0.0 (1) &  0.227 $\pm$ 0.0 (1) &  0.531 $\pm$ 0.0 (1) &  12004.0 $\pm$ 0.0 (1) &    703241.0 $\pm$ 0.0 (1) &    - \\
Independent Models   &  0.792 $\pm$ 0.0 (1) &  0.543 $\pm$ 0.0 (1) &  0.543 $\pm$ 0.0 (1) &  10000.0 $\pm$ 0.0 (1) &  17581025.0 $\pm$ 0.0 (1) &    - \\
NAS-D                &  0.792 $\pm$ 0.0 (1) &  0.597 $\pm$ 0.0 (1) &  0.597 $\pm$ 0.0 (1) &  65892.0 $\pm$ 0.0 (1) &  11972565.0 $\pm$ 0.0 (1) &    - \\
NAS-S beam=1         &  0.792 $\pm$ 0.0 (1) &  0.598 $\pm$ 0.0 (1) &  0.598 $\pm$ 0.0 (1) &  17346.0 $\pm$ 0.0 (1) &  14418814.0 $\pm$ 0.0 (1) &    - \\
NAS-S full           &                    - &                    - &                    - &                      - &                         - &    - \\
New-head finetune    &  0.792 $\pm$ 0.0 (1) &  0.238 $\pm$ 0.0 (1) &  0.528 $\pm$ 0.0 (1) &  11864.0 $\pm$ 0.0 (1) &    718721.0 $\pm$ 0.0 (1) &    - \\
New-head freeze      &  0.792 $\pm$ 0.0 (1) &  0.371 $\pm$ 0.0 (1) &  0.371 $\pm$ 0.0 (1) &   9344.0 $\pm$ 0.0 (1) &    718721.0 $\pm$ 0.0 (1) &    - \\
New-leg finetune     &  0.792 $\pm$ 0.0 (1) &   0.21 $\pm$ 0.0 (1) &  0.499 $\pm$ 0.0 (1) &  12280.0 $\pm$ 0.0 (1) &    715169.0 $\pm$ 0.0 (1) &    - \\
New-leg freeze       &  0.792 $\pm$ 0.0 (1) &  0.327 $\pm$ 0.0 (1) &  0.327 $\pm$ 0.0 (1) &  10252.0 $\pm$ 0.0 (1) &    715169.0 $\pm$ 0.0 (1) &    - \\
Online EWC           &  0.792 $\pm$ 0.0 (1) &  0.236 $\pm$ 0.0 (1) &  0.509 $\pm$ 0.0 (1) &  12820.0 $\pm$ 0.0 (1) &   2102463.0 $\pm$ 0.0 (1) &    - \\
PNN                  &                    - &                    - &                    - &                      - &                         - &    - \\

\bottomrule


\caption{\label{tab:res-long-25}Results in the long evaluation stream composed of 25 tasks.}
\end{tabular}

\end{center}
\end{table}

==> tables/stream_interferenceReset.tex <==
\begin{table}[]
\begin{center}
\begin{tabular}{llllllll}
\hline
                          & \multicolumn{1}{c}{$T_1$} & \multicolumn{1}{c}{$T_2$} & \multicolumn{1}{c}{$T_3$} & \multicolumn{1}{c}{$T_4$} & \multicolumn{1}{c}{$T_1+$}  \\ \hline
\textbf{Dataset}          & Cifar-10                   & MNIST                     & DTD                       & Fashion-MNIST             & Cifar-10                  \\
\textbf{\# Train samples} & 400                        & 400                       & 400                       & 400                       & 4000                      \\
\textbf{\# Val samples}   & 200                       & 200                      & 200                      & 200                      & 2000                       \\ \hline
\end{tabular}
\caption{\label{tab:stream-inter-reset}Details of the
  $\mathcal{S}^{\mbox{+}}$ stream used for evaluating the interference
  when a new version of a task arises with an order of magnitude more
  data.}
\end{center}
\end{table}


==> tables/stream_interferenceSimple.tex <==
\begin{table}[]
\begin{center}
\begin{tabular}{llllll}
\hline
                          & \multicolumn{1}{c}{$T_1$} & \multicolumn{1}{c}{$T_2$} & \multicolumn{1}{c}{$T_3$} & \multicolumn{1}{c}{$T_4$} & \multicolumn{1}{c}{$T_5*$} \\ \hline
\textbf{Dataset}          & MNIST                     & DTD                       & Fashion-MNIST             & SVHN                      & Cifar-10                   \\
\textbf{\# Train samples} & 400                       & 400                      & 400                       & 400                       & 4000                        \\
\textbf{\# Val samples}   & 200                       & 200                       & 200                       & 200                       & 2000                        \\ \hline
\end{tabular}
\caption{\label{tab:stream-interA}Details of the stream used for evaluating the interference property.}
\end{center}
\end{table}

==> tables/stream_transferInputTrans.tex <==
\begin{table}[]
\begin{center}
\begin{tabular}{lllllll}
\hline
                          & \multicolumn{1}{c}{$T_1$} & \multicolumn{1}{c}{$T_2$} & \multicolumn{1}{c}{$T_3$} & \multicolumn{1}{c}{$T_4$} & \multicolumn{1}{c}{$T_5$} & \multicolumn{1}{c}{$T_1'$} \\ \hline
\textbf{Dataset}          & MNIST                   & Cifar-10                     & DTD                       & Fashion-MNIST             & SVHN                      & MNIST                   \\
\textbf{\# Train samples} & 1000                       & 400                       & 400                       & 400                       & 400                       & 100                        \\
\textbf{\# Val samples}   & 500                       & 200                      & 200                      & 200                      & 200                      & 50                       \\ \hline
\end{tabular}
\caption{\label{tab:stream-remember-transfer-input-trans}Details of the stream used for evaluating the transfer property with input perturbation.}
\end{center}
\end{table}

==> tables/stream_transferRemember.tex <==
\begin{table}[]
\begin{center}
\begin{tabular}{lllllll}
\hline
                          & \multicolumn{1}{c}{$T_1$} & \multicolumn{1}{c}{$T_2$} & \multicolumn{1}{c}{$T_3$} & \multicolumn{1}{c}{$T_4$} & \multicolumn{1}{c}{$T_5$} & \multicolumn{1}{c}{$T_1^-$} \\ \hline
\textbf{Dataset}          & Cifar-10                   & MNIST                     & DTD                       & Fashion-MNIST             & SVHN                      & Cifar-10                   \\
\textbf{\# Train samples} & 4000                       & 400                       & 400                       & 400                       & 400                       & 400                        \\
\textbf{\# Val samples}   & 2000                       & 200                      & 200                      & 200                      & 200                      & 200                       \\ \hline
\end{tabular}
\caption{\label{tab:stream-remember-trans}Details of the stream used for evaluating the transfer property.}
\end{center}
\end{table}

==> tables/task-detail-2725.tex <==
\begin{tabular}{llllll}
\toprule
{} &        Dataset &                                            Classes &  # Train &  # Val &  # Test \\
\textbf{Task id} &                &                                                    &          &        &         \\
\midrule
\textbf{0      } &          mnist &                                    [6, 3, 7, 5, 0] &       25 &     75 &    4830 \\
\textbf{1      } &           svhn &                                    [2, 1, 9, 0, 7] &       25 &     75 &    5000 \\
\textbf{2      } &           svhn &                                    [2, 0, 6, 1, 5] &     5000 &  12500 &    5000 \\
\textbf{3      } &           svhn &                                    [1, 5, 0, 7, 4] &       25 &     75 &    5000 \\
\textbf{4      } &  fashion-mnist &  [T-shirt/top, Pullover, Trouser, Sandal, Sneaker] &       25 &     75 &    5000 \\
\textbf{5      } &  fashion-mnist &  [Shirt, Ankle boot, Sandal, Pullover, T-shirt/... &     5000 &  12500 &    5000 \\
\textbf{6      } &           svhn &                                    [3, 1, 7, 6, 9] &       25 &     75 &    5000 \\
\textbf{7      } &       cifar100 &       [spider, maple_tree, tulip, leopard, lizard] &       25 &     75 &     500 \\
\textbf{8      } &        cifar10 &           [frog, automobile, airplane, cat, horse] &       25 &     75 &    5000 \\
\textbf{9      } &  fashion-mnist &    [Ankle boot, Bag, T-shirt/top, Shirt, Pullover] &       25 &     75 &    5000 \\
\textbf{10     } &          mnist &                                    [4, 8, 7, 6, 3] &     5000 &  12500 &    4914 \\
\textbf{11     } &        cifar10 &              [automobile, truck, dog, horse, deer] &     5000 &  12500 &    5000 \\
\textbf{12     } &       cifar100 &          [sea, forest, bear, chimpanzee, dinosaur] &       25 &     75 &     500 \\
\textbf{13     } &          mnist &                                    [3, 2, 9, 1, 7] &       25 &     75 &    5000 \\
\textbf{14     } &  fashion-mnist &           [Bag, Ankle boot, Trouser, Shirt, Dress] &       25 &     75 &    5000 \\
\textbf{15     } &        cifar10 &                 [frog, cat, horse, airplane, deer] &       25 &     75 &    5000 \\
\textbf{16     } &        cifar10 &              [bird, frog, ship, truck, automobile] &     5000 &  12500 &    5000 \\
\textbf{17     } &           svhn &                                    [0, 4, 7, 5, 6] &     5000 &  12500 &    5000 \\
\textbf{18     } &          mnist &                                    [6, 5, 9, 4, 8] &     5000 &  12500 &    4806 \\
\textbf{19     } &          mnist &                                    [8, 5, 6, 4, 9] &     5000 &  12500 &    4806 \\
\textbf{20     } &       cifar100 &          [sea, pear, house, spider, aquarium_fish] &       25 &     75 &     500 \\
\textbf{21     } &       cifar100 &            [kangaroo, ray, tank, crocodile, table] &     2250 &   1250 &     500 \\
\textbf{22     } &       cifar100 &                  [trout, rose, pear, lizard, baby] &       25 &     75 &     500 \\
\textbf{23     } &           svhn &                                    [3, 2, 8, 1, 5] &     5000 &  12500 &    5000 \\
\textbf{24     } &       cifar100 &           [skyscraper, bear, rocket, tank, spider] &       25 &     75 &     500 \\
\textbf{25     } &       cifar100 &     [telephone, porcupine, flatfish, plate, shrew] &     2250 &   1250 &     500 \\
\textbf{26     } &       cifar100 &          [lawn_mower, crocodile, tiger, bed, bear] &       25 &     75 &     500 \\
\textbf{27     } &           svhn &                                    [3, 7, 1, 5, 6] &       25 &     75 &    5000 \\
\textbf{28     } &  fashion-mnist &      [Ankle boot, Sneaker, T-shirt/top, Coat, Bag] &     5000 &  12500 &    5000 \\
\textbf{29     } &          mnist &                                    [6, 9, 0, 3, 7] &     5000 &  12500 &    4938 \\
\textbf{30     } &        cifar10 &               [automobile, truck, deer, bird, dog] &       25 &     75 &    5000 \\
\textbf{31     } &        cifar10 &            [dog, airplane, frog, deer, automobile] &     5000 &  12500 &    5000 \\
\textbf{32     } &           svhn &                                    [1, 9, 5, 3, 6] &     5000 &  12500 &    5000 \\
\textbf{33     } &       cifar100 &   [whale, orange, chimpanzee, poppy, sweet_pepper] &       25 &     75 &     500 \\
\textbf{34     } &       cifar100 &               [worm, camel, bus, keyboard, spider] &       25 &     75 &     500 \\
\textbf{35     } &  fashion-mnist &      [T-shirt/top, Coat, Ankle boot, Shirt, Dress] &       25 &     75 &    5000 \\
\textbf{36     } &        cifar10 &                      [dog, deer, ship, truck, cat] &       25 &     75 &    5000 \\
\textbf{37     } &        cifar10 &                   [cat, dog, airplane, ship, deer] &     5000 &  12500 &    5000 \\
\textbf{38     } &           svhn &                                    [7, 6, 4, 2, 9] &       25 &     75 &    5000 \\
\textbf{39     } &          mnist &                                    [9, 7, 1, 3, 2] &       25 &     75 &    5000 \\
\textbf{40     } &       cifar100 &        [mushroom, butterfly, bed, boy, motorcycle] &       25 &     75 &     500 \\
\textbf{41     } &  fashion-mnist &        [Shirt, Pullover, Bag, Sandal, T-shirt/top] &       25 &     75 &    5000 \\
\textbf{42     } &       cifar100 &           [rabbit, bear, aquarium_fish, bee, bowl] &       25 &     75 &     500 \\
\textbf{43     } &  fashion-mnist &       [Coat, T-shirt/top, Pullover, Shirt, Sandal] &       25 &     75 &    5000 \\
\textbf{44     } &  fashion-mnist &             [Pullover, Dress, Coat, Shirt, Sandal] &       25 &     75 &    5000 \\
\textbf{45     } &          mnist &                                    [3, 9, 7, 6, 4] &       25 &     75 &    4940 \\
\textbf{46     } &        cifar10 &                [deer, bird, dog, automobile, frog] &       25 &     75 &    5000 \\
\textbf{47     } &           svhn &                                    [8, 7, 1, 0, 4] &       25 &     75 &    5000 \\
\textbf{48     } &       cifar100 &       [forest, skunk, poppy, bridge, sweet_pepper] &     2250 &   1250 &     500 \\
\textbf{49     } &       cifar100 &   [caterpillar, can, motorcycle, rabbit, wardrobe] &       25 &     75 &     500 \\
\textbf{50     } &       cifar100 &        [trout, mountain, kangaroo, pine_tree, bee] &       25 &     75 &     500 \\
\textbf{51     } &       cifar100 &             [clock, fox, castle, bus, willow_tree] &       25 &     75 &     500 \\
\textbf{52     } &        cifar10 &                  [cat, airplane, dog, ship, truck] &       25 &     75 &    5000 \\
\textbf{53     } &          mnist &                                    [9, 7, 8, 1, 5] &       25 &     75 &    4866 \\
\textbf{54     } &  fashion-mnist &           [Bag, T-shirt/top, Sandal, Shirt, Dress] &       25 &     75 &    5000 \\
\textbf{55     } &  fashion-mnist &       [Sneaker, Ankle boot, Coat, Sandal, Trouser] &     5000 &  12500 &    5000 \\
\textbf{56     } &          mnist &                                    [1, 4, 3, 9, 7] &       25 &     75 &    4982 \\
\textbf{57     } &        cifar10 &               [truck, automobile, frog, ship, dog] &       25 &     75 &    5000 \\
\textbf{58     } &          mnist &                                    [7, 2, 8, 5, 4] &       25 &     75 &    4848 \\
\textbf{59     } &          mnist &                                    [2, 8, 9, 1, 7] &     5000 &  12500 &    4974 \\
\textbf{60     } &           svhn &                                    [9, 5, 1, 8, 6] &       25 &     75 &    5000 \\
\textbf{61     } &          mnist &                                    [1, 8, 7, 4, 5] &       25 &     75 &    4848 \\
\textbf{62     } &        cifar10 &           [truck, dog, bird, automobile, airplane] &       25 &     75 &    5000 \\
\textbf{63     } &          mnist &                                    [8, 4, 3, 7, 6] &       25 &     75 &    4914 \\
\textbf{64     } &           svhn &                                    [3, 5, 7, 2, 1] &       25 &     75 &    5000 \\
\textbf{65     } &       cifar100 &                   [otter, camel, bee, road, poppy] &       25 &     75 &     500 \\
\textbf{66     } &           svhn &                                    [4, 2, 1, 8, 7] &       25 &     75 &    5000 \\
\textbf{67     } &          mnist &                                    [3, 7, 6, 8, 9] &       25 &     75 &    4932 \\
\textbf{68     } &  fashion-mnist &        [Pullover, Sneaker, Trouser, Dress, Sandal] &       25 &     75 &    5000 \\
\textbf{69     } &           svhn &                                    [5, 0, 7, 2, 3] &       25 &     75 &    5000 \\
\textbf{70     } &           svhn &                                    [9, 6, 2, 4, 8] &       25 &     75 &    5000 \\
\textbf{71     } &          mnist &                                    [7, 1, 2, 0, 6] &       25 &     75 &    4938 \\
\textbf{72     } &        cifar10 &             [dog, automobile, ship, airplane, cat] &       25 &     75 &    5000 \\
\textbf{73     } &          mnist &                                    [0, 7, 6, 2, 4] &       25 &     75 &    4920 \\
\textbf{74     } &        cifar10 &                  [bird, deer, airplane, dog, ship] &       25 &     75 &    5000 \\
\textbf{75     } &       cifar100 &   [mountain, bicycle, caterpillar, spider, possum] &       25 &     75 &     500 \\
\textbf{76     } &           svhn &                                    [8, 3, 4, 0, 6] &       25 &     75 &    5000 \\
\textbf{77     } &           svhn &                                    [1, 5, 9, 0, 8] &       25 &     75 &    5000 \\
\textbf{78     } &       cifar100 &          [can, dolphin, house, pickup_truck, crab] &       25 &     75 &     500 \\
\textbf{79     } &       cifar100 &   [squirrel, possum, crocodile, mountain, hamster] &       25 &     75 &     500 \\
\textbf{80     } &          mnist &                                    [7, 0, 1, 6, 2] &       25 &     75 &    4938 \\
\textbf{81     } &  fashion-mnist &      [T-shirt/top, Dress, Trouser, Shirt, Sneaker] &       25 &     75 &    5000 \\
\textbf{82     } &        cifar10 &             [cat, frog, automobile, dog, airplane] &       25 &     75 &    5000 \\
\textbf{83     } &        cifar10 &                [automobile, cat, dog, ship, horse] &       25 &     75 &    5000 \\
\textbf{84     } &       cifar100 &               [cup, otter, orchid, kangaroo, rose] &       25 &     75 &     500 \\
\textbf{85     } &          mnist &                                    [1, 5, 7, 2, 9] &       25 &     75 &    4892 \\
\textbf{86     } &           svhn &                                    [6, 5, 3, 2, 7] &       25 &     75 &    5000 \\
\textbf{87     } &        cifar10 &                       [dog, deer, cat, frog, bird] &       25 &     75 &    5000 \\
\textbf{88     } &          mnist &                                    [6, 2, 5, 9, 4] &       25 &     75 &    4832 \\
\textbf{89     } &       cifar100 &                  [pear, rocket, sea, road, orange] &       25 &     75 &     500 \\
\textbf{90     } &           svhn &                                    [0, 8, 4, 6, 1] &       25 &     75 &    5000 \\
\textbf{91     } &        cifar10 &                    [truck, horse, ship, deer, dog] &       25 &     75 &    5000 \\
\textbf{92     } &          mnist &                                    [5, 8, 6, 4, 3] &       25 &     75 &    4806 \\
\textbf{93     } &           svhn &                                    [2, 6, 3, 4, 1] &       25 &     75 &    5000 \\
\textbf{94     } &  fashion-mnist &        [Bag, Trouser, Sneaker, Ankle boot, Sandal] &       25 &     75 &    5000 \\
\textbf{95     } &           svhn &                                    [7, 9, 1, 5, 8] &       25 &     75 &    5000 \\
\textbf{96     } &       cifar100 &            [lamp, otter, skyscraper, sea, raccoon] &       25 &     75 &     500 \\
\textbf{97     } &       cifar100 &                 [clock, flatfish, snake, can, man] &       25 &     75 &     500 \\
\textbf{98     } &           svhn &                                    [6, 3, 0, 8, 7] &       25 &     75 &    5000 \\
\textbf{99     } &  fashion-mnist &             [Shirt, Coat, Dress, Sandal, Pullover] &       25 &     75 &    5000 \\
\bottomrule
\end{tabular}

